A Massive Scale Semantic Similarity Dataset of Historical English

A diversity of tasks use language models trained on semantic similarity data. While there are a variety of datasets that capture semantic similarity, they are either constructed from modern web data or are relatively small datasets created in the past decade by human annotators. This study utilizes a novel source, newly digitized articles from off-copyright, local U.S. newspapers, to assemble a massive-scale semantic similarity dataset spanning 70 years from 1920 to 1989 and containing nearly 400M positive semantic similarity pairs. Historically, around half of articles in U.S. local newspapers came from newswires like the Associated Press. While local papers reproduced articles from the newswire, they wrote their own headlines, which form abstractive summaries of the associated articles. We associate articles and their headlines by exploiting document layouts and language understanding. We then use deep neural methods to detect which articles are from the same underlying source, in the presence of substantial noise and abridgement. The headlines of reproduced articles form positive semantic similarity pairs. The resulting publicly available HEADLINES dataset is significantly larger than most existing semantic similarity datasets and covers a much longer span of time. It will facilitate the application of contrastively trained semantic similarity models to a variety of tasks, including the study of semantic change across space and time.

==> dates.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{count_graph.png}
    \caption{Semantic similarity pairs by year.}
    \label{fig:dates}
\end{figure}


==> wire_clu_data.tex <==
\begin{table}[t]
    \centering
    %\resizebox{\linewidth}{!}{
    \begin{threeparttable}
        \begin{tabular}{lccccc}
        \toprule
             &  Positives & Negative  & Reproduced  & Singleton & Total    \\
             & Pairs & Pairs & Articles & Articles & Articles \\
        \midrule
        \textbf{Training Data} \\
       Training	&	36,291	&	37,637	&	891	&	--	&	7,728 \\
Validation	&	3,042	&	3,246	&	20	&	--	&	283 \\
\midrule
\textbf{Full Day Evaluation}	&		&		&		&		&	\\
Validation	&	28,547	&	12,409,031	&	447	&	2,162	&	4,988 \\
Test	&	54,996	&	100,914,159	&	1,236	&	8,046	&	14,211 \\
\midrule
\textbf{Full Dataset}	&	122,876	&	113,364,073	&	2,594	&	10,208 	&	27,210 \\
        \bottomrule 
    \end{tabular}
    \end{threeparttable}
   %}
    \caption{This table provides summary statistics from the \texttt{NEWS-COPY} dataset, decomposed into the training sample and the full day evaluation data.}
    \label{wire_clu_sumstat}
    \vspace{-5mm}
\end{table}
